Survey and Taxonomy of Adversarial Reconnaissance Techniques

Adversaries are often able to penetrate networks and compromise systems by exploiting vulnerabilities in people and systems. The key to the success of these attacks is information that adversaries collect throughout the phases of the cyber kill chain. We summarize and analyze the methods, tactics, and tools that adversaries use to conduct reconnaissance activities throughout the attack process. First, we discuss what types of information adversaries seek, and how and when they can obtain this information. Then, we provide a taxonomy and detailed overview of adversarial reconnaissance techniques. The taxonomy introduces a categorization of reconnaissance techniques based on the source as third-party, human-, and system-based information gathering. This paper provides a comprehensive view of adversarial reconnaissance that can help in understanding and modeling this complex but vital aspect of cyber attacks as well as insights that can improve defensive strategies, such as cyber deception.

==> sections/lesson.tex <==
%________________________________________________
%%% -------------  NEW SECTION  ------------- %%%
%------------------------------------------------
% \section{Lessons Learned} \label{sec: Lessons-Learned}
% \subsection{Effectiveness of Reconnaissance}
% \Aron{This paragraph is very high level and does not seem to build on the taxonomy (or any other contributions of the paper). So, it would fit better into the introduction then lessons learned. If we cannot build it on the contributions of this paper, then we should probably omit it.}
% Reconnaissance provides potential inputs to adversaries for planning the next steps and maximizes benefits. No system is safe as every technology is vulnerable by design. For example, there must be a bypassing way if we forget the pattern or password of our handheld devices. Adversaries identify these vulnerabilities of devices from different vendors and develop tools to remotely exploit them. But before exploiting those vulnerabilities, they need information in detail about the devices, networks, platforms, services, and applications used by the target. Reconnaissance phases take days to months or years intending to gather as much information as adversaries can have about the target. The collected information is used thereby to map common vulnerabilities and exposures (CVE) with the tools they have in their collection. Most of the tools are crafted by adversaries to initiate a zero-day attack with remaining undetected in the system. While crafting tools or buying necessary parts of APT through the dark web, the gathered information from the Reconnaissance phases play a vital role.


% \subsection{Cyber Security against Reconnaissance}
\section{Reconnaissance Mitigation and Prevention
% \Jaime{Would reorder to parallel sec 3; social engineering (user), target (application/host), network}\Aron{We can discuss this. We probably don't want to re-organize Section 5 entirely; but it would be nice to structure some of its subsections similar to Section 3.}
}\label{sec: recon-mitigate}
 
% \Aron{What do you mean by `defensive measurement'? Did you mean `defensive measure'?}

Defensive measures against the reconnaissance techniques differ from one another based on the approaches, target people or platform, and the tools adversaries use. Defenders can attempt to mitigate a few reconnaissance techniques while in other cases mitigation and prevention measures are not effective. For example, it is quite difficult to prevent internet footprinting as organizations keep exposing themselves through marketing. Besides, information exposure largely depends on the people working within the organization and they are equally responsible to keep confidential information safe and out of the reach of adversaries. Social engineering is a psychological game between two parties and one is the ultimate winner. Social engineering has no technical defensive measures and only sufficient training and security awareness can mitigate it at large. Network scanning techniques are a bit cautious from the adversary's perspective. Therefore, defenders can utilize enforced firewall rules, intrusion detection and prevention measures, cyber deception, and moving target defense technologies to mitigate and prevent the effectiveness of scanning techniques. Local discoveries have limited
%\Aron{Honeytokens?} 
preventive measures as 
% \Aron{What does `it' refer to?}
discovery involves obtaining local information in a compromised host through overwriting system configurations and basic command-line tools and techniques. 
Regardless of the different techniques utilized by adversaries, organizations take certain measures to defend their resources. Defense involves physical precautions, use of firewalls and intrusion detection systems (e.g., host or network-based IDS), enforcement of security training to employees, secure network administration, zoning, and other best practices. Apart from the traditional security measures, both academia and the industry is adapting to modern defensive techniques such as deception and moving target defenses (MTD) intending to deceive the attacker and make the search or operational space more complex.

Figure~\ref{fig:attack_surface} refers to the attack process from the adversary's perspective and the defensive measures from the defender's perspective. The figure depicts how adversaries approach based on the external and internal reconnaissance and in contrast, what defensive measures organizations can utilize.

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=\textwidth, height=\textheight,keepaspectratio]{images/Recon_mitigate.pdf}
    \caption{Adversary's Surface vs. Defender's Surface}
    \label{fig:attack_surface}
\end{figure*}



\subsection{Reconnaissance Detection}

In order to mitigate and limit adversarial reconnaissance, defenders are required to detect the actions, behaviors, and patterns of these techniques. \emph{Target footprinting} techniques can rarely be detected though as it is passive and other people (e.g., employees, network administrator, business competitor, job seekers) can look for publicly available organization information as well. The only way to mitigate target footprinting is understanding the privacy level (confidential or public) of data before publishing or posting in a data source (websites, documents, magazines, etc.).

% \subsubsection{Social Engineering Detection and Prevention}
\emph{Social engineering} techniques are combination of different confidence tricks that are difficult for the defender (a person or a group of people) to identify against a skilled attacker. However, effective understanding of the context in terms of the requester identity (authority level, credibility, previous existence, verifiable, etc.) and data (sensitivity, necessity to provide, public/private domain, etc.) can help to identify such attacks at large~\cite{mouton2015social}. Phishing is one of most common form of social engineering and according to Nicholson et al.,\ defender person can identify a phishing email better when they have more attention to the sender's details~\cite{nicholson2017can}. However, people who make quick decisions are prone to fall victim to the phishing emails. Sawa et al.\ utilizes natural language processing to identify typical suspicious questions and commands used by adversaries~\cite{sawa2016detection}. Ahmed et al.\ differentiates phishing URLs from regular ones by developing an algorithm that checks for URL length, number of ``//'' appear in the URL, if contains ``@'' or not, and if there is ``-'' in prefix or suffix~\cite{ahmed2016real}. Apart from these detection and mitigation techniques, mobile users can take typical measures such as content filtering, blacklisting, and whitelisting of web addresses to tackle phishing, smishing, and vishing~\cite{shahriar2015mobile}.
% Sandouka et al.\ utilized neural network to detect social engineering based on feature extraction from benchmark data (attributes/words/phrases of a phone call)~\cite{sandouka2009social}.


% \subsubsection{Scanning Detection and Prevention}
\emph{Network scanning} techniques are performed frequently from an external network and it is more robust within the internal network once an internal host is compromised. System and network administrators are required to protect the organization network from these scans because this is how adversaries get to know about active hosts, ports, and vulnerabilities. However, recognizing the scans performed by adversaries are typically a strenuous task for administrators and adversaries have been innovating new strategies to avoid detection.
Bhuyan et al.\ proposed two approaches towards detecting severe port scans such as \emph{single-source} and \emph{distributed} port detection~\cite{bhuyan2011surveying}. The single source scan can be detected at \emph{flow-level} or \emph{packet-level}. Authors have also categorized single source scan detection as \emph{algorithmic approaches} that use hypothesis testing and probabilistic models to detect the scans (e.g., detection using network packet-based activity graph~\cite{staniford1996grids}, anomaly-based detection~\cite{kim2004detecting,bhuyan2017network}), \emph{threshold-based approaches} that use a fixed-size time window to detect how many unique IP addresses have already been contacted by the host (e.g., checking number of SYN packets over a time~\cite{roesch1999snort}, number of destinations contacted by a single source~\cite{paxson1999bro}, time-based flow size distribution~\cite{zhang2009novel}), \emph{soft-computing approaches} that emphasize flexible information processing to trace the scan origin (e.g., detection based on learning from past histories of open ports~\cite{chen2009novel}, \cite{liu2008network}), \emph{rule-based approaches} that utilize stored rules in the knowledge-base to detect and prevent typical scans (e.g., abnormal traffic control framework~\cite{kim2008slow}), and \emph{visual approaches} that leverage visualization to detect a particular network event like scanning (e.g., visualizing patterns of scan generated by Nmap, Nessus, etc.~\cite{conti2004passive}). In contrast, authors claimed that distributed scans can be tracked at \emph{packet-level} and \emph{alert-level}. Different algorithmic, soft-computing, and visual approaches in a distributed mode, and clustering-based methods can be used to detect distributed scans~\cite{robertson2003surveillance,staniford2002practical,gates2006co}.

Kim et al.\ proposed a scanning detection mechanism based on fuzzy logic and a stepwise policy (decreasing network bandwidth $\rightarrow$ discarding packets)~\cite{kim2008slow}. Their framework had an intrusion detection module consisted of a ``packet analysis'' and an ``intrusion analysis'' sub-modules that analyze the network packets using fuzzy logic and inspects intrusion respectively. The intrusion prevention module included a ``packet filtering'' sub-module that blocks abnormal packets and a ``queue assignment'' sub-module that narrows the bandwidth if a series of packets are found suspicious.  
Scanning using botnets make it more convenient for adversaries to hide the true identity and the origin of an attack. Botnets can recruit vulnerable hosts to spread and launch scanning attacks. Botnets are robust in a large scale attack and adversaries can execute commands through a C\&C channel. As these bots are used to perform several scanning algorithms (e.g., uniform, non-uniform, localized), it is necessary to detect botnet commands and compromised host. Gu et al.\ utilized statistical analysis to detect spatial-temporal correlation and similarity with the previous real-world botnets so that they can capture the engagement by analyzing the network traffic~\cite{gu2008botsniffer}.


Vulnerability scan detection is typically strenuous in a network if it is limited to passive banner grabbing. However, active scanning can be detected in a server if adversaries leave logs behind. Seyyar et al.\ proposed to detect potential web vulnerability scan by looking into the access log files of different web servers (e.g., Apache, IIS)~\cite{seyyar2018detection}. The rule-based detection works by examining the past recorded logs using existing vulnerability scanners and analyzing suspicious activities. 

\emph{Local discovery} techniques are performed when adversaries already have access to the system and if privileges are escalated, there is less chance to detect and mitigate the reconnaissance. However, using host-based intrusion detection techniques and security softwares (antivirus or firewall) can be efficient against inexperienced attackers.


\subsection{Cyber Deception and Moving Target Defense}
The traditional mechanism against reconnaissance lies in customized network design, firewalls, network address translations (NAT), DMZ, subnetting, etc. However, traditional network management does not guarantee security due to misconfigurations, constant scenario changes, and other human errors. Therefore, next-generation concepts such as \emph{Cyber Deception} and \emph{Moving Target Defense} (MTD) have evolved in the network security scenario; bringing more features to mitigate adversarial scanning and discoveries.

Cyber deception and MTD adapts to the adversary's behavior and manipulate their behavior by creating static or dynamic deception and diversion. Wang et al.\ differentiate cyber deception from MTD 
% \Aron{This sentence structure is not clear. Wang et al. are focusing on static...?}
based on static pre-configuration and misdirection by providing misleading information while MTD focuses on dynamic approaches by increasing complexity and diversity on the fly \cite{wang2018cyber}. Crouse et al. elaborate the differentiation by providing examples for each approach: deception includes network masking, decoying, mimicking, and inventing (honeypots); on the other hand, MTD includes dynamic network shuffle, configuration adaptation, and evolution, and Address Space Layout Randomization (ASLR) \cite{crouse2015probabilistic}. ASLR involves random rearrangement of address spaces positions of a process in the memory to prevent successful code or script execution. 
% According to \Aron{Which authors?}authors,
Crouse et al.\ also claimed that, reconnaissance defense using deception or movement costs the attacker more than the defender making the defenses potentially successful. 

Han et al.\ have surveyed and listed several deception techniques that are able to mitigate, detect or prevent adversarial reconnaissance~\cite{han2018deception}. The list includes deceptive topology, OS obfuscation, traffic forging, decoy services, etc.\ as network-layer deception; decoy computation, multi-layer deception, fake honeypots, honey-permission, etc.\ as system-level deception; software decoys, honey-patches, shadow honeypots, honey-URL, honey-accounts etc.\ as application-level deception; and honey-passwords, honey-encryption, honey-accounts, honey-files, honey-profiles and webpages, etc.\ as data-level deception.
The earlier stage of cyber deception grew mostly from the tactics of military deceptions. Trassare et al.\ proposed a proof-of-concept network to deceive the UDP-based ``traceroute'' query by shunting the incoming packet to a deceptive topology~\cite{trassare2013technique}.
Deploying honeypots in the network can create misdirection and eventually can detect intrusion. However, Wang et al.\ claim that botnet attacks are very common nowadays and adversaries are capable of identifying the honeypot nodes in both centralized and peer-to-peer (P2P) botnets~\cite{wang2010honeypot}. Therefore, researchers have come with different solutions to address this problem. Challoo et al.\ experimented to detect adversarial botnets using honeypots by differentiating between the infected honeypot and the uninfected one~\cite{challoo2011detection}. On the other hand, Al-Hakbani et al.\ utilize peer lists and vulnerabilities information to prevent the Advanced Two-Stage Reconnaissance Worm (ASTRW) by remotely controlling the infected hosts~\cite{al2015avoiding}.

Not only the academia but also the global industry is adapting to the deception technologies. According to the Global cyber deception report of 2019 \cite{GlobalCy21:online}, a few of the key players in the market who already have developed security systems adapting to deception technologies are Rapid7\footnote{\url{https://www.rapid7.com/products/insightidr/features/deception-technology/}},
% ~\cite{Deceptio27:online}, 
LogRhythm\footnote{\url{https://logrhythm.com/}},
% ~\cite{LogRhyth19:online}, 
Trapx Security (DeceptionGrid\footnote{\url{https://trapx.com/product/}}),
% ~\cite{productT7:online}), 
Attivo Networks\footnote{\url{https://attivonetworks.com/deception-based-threat-detection/}},
% ~\cite{Deceptio87:online}, 
Illusive Networks\footnote{\url{https://www.illusivenetworks.com/}},
% ~\cite{NetworkS97:online}, 
Smokescreen Technologies\footnote{\url{https://www.smokescreen.io/}},
% ~\cite{Smokescr45:online}, 
Acalvio Technologies\footnote{\url{https://www.acalvio.com/}},
% ~\cite{AcalvioS14:online}, 
etc.

\subsubsection{Software-Defined Networking in Deception and MTD}
% \Aron{what do you mean by `Movement'? MTD?}
Software-Defined Networking (SDN) has been utilized well in both deception and movement strategies.
% \Shanto{I'll add a few more} 
Shimanaka et al.\ proposed a system that creates an identically configured network for deceiving adversarial reconnaissance~\cite{shimanaka2019cyber}. The system was designed intending to minimize further compromise once intrusion is detected by redirecting all traffic from the operational network (O-net) to deception network (D-net).
SDN can deceive adversaries by simulating virtual networks and can defend from potential insider reconnaissance as well. Achleitner et al.\ developed  a reconnaissance deception system (RDS) that delays the adversarial scanning and invalidates their already collected information over time~\cite{achleitner2016cyber}~\cite{achleitner2017deceiving}. The simulation can mitigate network reconnaissance techniques such as vulnerable host scanning by APTs. With the evolve of network deception techniques utilizing SDN, Robertson et al.\ developed \emph{CINDAM} that creates modified per-host view to make the network topology more unpredictable~\cite{robertson2015cindam}. CINDAM was cost-effective and achieved this deception without affecting any visible performance issue in the internal network. Later, Chiang et al.\ developed an adaptive cyber deception system entitled \emph{ACyDS} that changes the network view of each host dynamically~\cite{chiang2016acyds}. To build the network deception more adaptive, Sugrim et al.\ proposes to combine deception and MTD; intending to present a \emph{dynamic virtual attack surface}~\cite{sugrim2018measuring}. This virtual surface features isolated view for each host, dynamic change of view, and large search space (subnets with large number of hosts). 

Wang et al.\ developed a method using SDN based MTD, Sniffer Reflector to prevent adversarial network reconnaissance. Sniffer Reflector simply creates an obfuscated view for adversaries to refrain them from obtaining the original result~\cite{wang2016moving}. Shi et al.\ developed another SDN-based MTD approach called CHAOS that features IP, ports, and fingerprint obfuscation to present the network environment more unpredictable~\cite{shi2017chaos}. As fingerprinting is severe within the internal network, Zhao et al. have developed a signal game utilizing the SDN-based fingerprint hopping (FPH) method to counter adversarial fingerprinting techniques \cite{zhao2017sdn}. To prevent scanning techniques, Wang et al. have proposed random domain name and address mutation (RDAM) that increases the address search space by dynamically changing or remapping the IP addresses in a network \cite{wang2017random}.





\subsubsection{Techniques and Components of Deception and MTD Deployment}
% \Aron{title mentions MTD, but all of the paragraphs are concerned with deception (not with MTD)}
Network virtualization and network function virtualization can easily be utilized to create dynamic views from each host, topology deception and creating large scaling search spaces using low-cost virtual machines. Both Deception and MTD targets to mislead adversaries by providing false information and direction within the network. Deception and MTD introduce different techniques and tools so far that are utilized by altering static and dynamic configurations in the network.

\paragraph{Deception and MTD Techniques}
Several deception and MTD techniques have been utilized to-date and researchers have been introducing new techniques for efficient deception/MTD-based defense. After SDN has been introduced, deploying these techniques have become easier. 
Deception techniques can be applied in different layers such as network layer, data layer, application layer and phases of the network system. 
The following deception techniques are appropriate for insider adversaries who have placed themselves in the network (on one or more hosts), using techniques such as social engineering, exploiting zero-day vulnerabilities, via drive-by downloads or by manual infection, etc.
% Here, we discuss a few deception/MTD deployment techniques implemented so far:

\begin{itemize}
    \item\textbf{Dynamic address translation (DAT):} 
    To make the overall address space of a network appear larger on-the-fly packet header rewriting can be used to hide the real host addresses which make the network search space big. DAT can be implemented by both hardware and software through the use of page tables, segment tables, region tables.  Additionally, allows different address spaces to share the same program or other data that is for read-only. The translation of the real underlying network’s address space into a significantly larger  address space increases the search space for adversarial scanners and invalidate their gathered information
\cite{achleitner2017deceiving,achleitner2016cyber}.

\item\textbf{Route alteration:}  By simulating virtual paths, multiple hops from a source to a destination host can be spanned \cite{achleitner2016cyber}. Which  can alter the topology of different network views so that a scanner will be unable to correctly conclude about the real network topology~\cite{borders2007openfire}.

\item\textbf{Address space randomization:}
The IP address space of the target network including both the real servers and the decoys can be shuffled~\cite{sun2016desir}. Although through reconnaissance, the attacker can create a blacklist of decoy IP addresses, this blacklist will not be valid after the next round of IP randomization, and the attacker has to start over the reconnaissance process.


\item\textbf{Forwarding ARP requests to deception server:}
ARP packet is an important part of the deception system. ARP requests are usually flooded into the network to discover hosts and match IP to MAC addresses. By including a deception server which can handle all ARP requests forwarded to it and sends the appropriate response packets which can ensure that hosts which are not supposed to be discovered stay hidden \cite{rowe2004model,achleitner2016cyber}.

\item\textbf{Resource obfuscation:}
Host-based (OS) obfuscation, ports, address space, and obfuscation based on decoys can mitigate internal recon by making the network more unpredictable~\cite{shi2017chaos}. Resource obfuscation through migration and dynamic mapping provide a complex large search space for adversaries.
\end{itemize}


\paragraph{Deception and MTD Components}
Several tools and components are considered useful in terms of delaying and preventing adversarial reconnaissance. These components effectively complement other well-known intrusion detection and prevention techniques as well. Moreover, it improves on the more conventional approaches that the security community has studied and implemented during the past 35 years\cite{wang2018cyber}. Here we discuss a few common tools used for cyber deception and MTD:

\subparagraph{Honeypots} Honeypots are 
% \Aron{what does PC stand for in this context?}
host machine frameworks intended to be attacked so that it helps network administrator to analyze the attack pattern without having any damage to other real network nodes. It can be used in different aspects of security such as prevention, detection, and information gathering. It is a tool that is flexible in nature and with applications in many areas of the network. There are two particular honeypot types:
  
\begin{itemize}
\item \textbf{High-interaction honeypot:} It simulates all aspects of an operating system. Via High Interaction honey pot attackers can gain full access to the system
\item \textbf{Low-interaction honeypots:} It can simulate only some parts, such as the network stack.Via low-interaction honeypots adversaries can simulate only services that cannot be exploited to get complete access to the system \cite{shulman2015compromised}.
\end{itemize}

The key advantage of using honeypots is to mislead adversaries to decoy systems and to detect an intrusion in a system or network. Besides, using honeypots the size of a search space and sparsity of real vulnerabilities can be increased. Apart from these, a deep examination of adversaries during and after exploitation of a honeypot can be analyzed~\cite{mokube2007honeypots} for considering further security measures. However, honeypots can be used as a launching platform to attack other hosts on different network~\cite{mokube2007honeypots}.

% \textbf{Advantages:}
% \begin{itemize}
%     \item[a)] Attackers can be distracted from more valuable machines on
% a network.
%     \item[b)] Early warning about new attack and exploitation trends can be monitored.
%     \item[c)] Increase the size of the search space and the sparsity of real vulnerabilities.
%     \item[d)] A deep examination of adversaries during and after exploitation of a honeypot can be analyzed \cite{mokube2007honeypots}.
% \end{itemize}

% \textbf{Disadvantages:}
% \begin{itemize}
%     \item[a)] They are worthless if not being attacked.
%     \item[b)] Can be used as a launching platform to attack other hosts on different
% network \cite{mokube2007honeypots}
% \end{itemize}
    

\subparagraph{Honeytools}
The prefix ``honey'' has been utilized to allude to a wide scope of methods that fuse the demonstration of deceiving in them. The fundamental thought behind the utilization of the prefix word ``honey'' in these methods is that they have to allure adversaries to interact with them.

    \begin{itemize}
    \item \textbf{Honeyfiles:} Honey files are bogus files and folders that make real files and folders indistinguishable from fake files and folders. After the attacker intrudes inside the network and compromises a machine, he can escalate his privilege into the next stage of an attack, where local emails, files, and folders are explored. Honey files (HFs) can play a deception role in this phase. Honeyfiles can be perfectly believable decoys or the modification of authenticating files to include some alteration in the function~\cite{provos2004virtual}.

    \item \textbf{Honeytokens:} This is similar to honey flies. These are fake data that attracts attacker to interact with the data, for example, DNS honey token is a complementary technique to honeypots. Whenever adversaries use “brute force” for common subdomains or attempt a zone transfer, DNS servers will try to identify interesting resources (e.g., sub-domains, servers) as part of their reconnaissance process. By creating a small number of fake DNS records on the authoritative DNS servers of the organization and by configuring them to initiate an alert when these specific records are requested; defenders can receive an early warning of DNS-related information-gathering attempts against their infrastructure. Another example, fake credit card numbers can be inserted into the repository within a network. IDS’s can be configured to watch the network if these are accessed then the notification of system compromised will be sent to defender~\cite{mokube2007honeypots}.
    
    \item \textbf{HoneyGen:} Honeygen is usually used to produce honeytokens automatically. HoneyGen produces honeytokens that are similar to the real data by deriving the characteristics and properties of real data. These honeytokens can be used to detect intrusions, data misuse and data leakage by adversaries. Honey tokens can be implemented among real tokens in the database and can be monitored to detect any activity associated with them~\cite{bercovitch2011honeygen}.
    
    \item\textbf{Honeywords:} Honeywords or honey-passwords are typical fake passwords, utilized to confuse adversaries in finding the difference between real and fake passwords when they crack a stolen hashed password file. Honey passwords are having multiple possible passwords for each account, only one of which is genuine~\cite{mokube2007honeypots}.
    
    \item\textbf{Honeyd:} A framework for virtual honeypots to simulate virtual computer systems at the network level. Honeyd can simulate the networking stack of various operating systems and able to provide arbitrary services for any number of virtual systems~\cite{provos2003honeyd}.

\end{itemize}

The usage of the above-mentioned tools can significantly increase the possibility of detecting potential attacks at different reconnaissance phases. 
% It allows defenders to mitigate a threat before the adversaries fulfill their objectives.
Combining these tools and techniques make reconnaissance, penetration and lateral movements further difficult for adversaries. However, the effectiveness of such measures against insiders is not measured yet as it is likely they know the use of these tools.
% Although it can be divided into many sections from the chosen paper application of  deception techniques to deceive attacker in the reconnaissance phase are described




% Figure~\ref{fig:attack_surface} represents how cyber deception can be utilized in terms of the scanning phase launched by an attacker.

%\begin{landscape}
% \begin{figure*}[!ht]
%     \centering
%     \includegraphics[width=\textwidth, height=\textheight,keepaspectratio]{images/Recon_mitigate.pdf}
%     \caption{Attacker's Surface vs Defender's Surface}
%     \label{fig:attack_surface}
% \end{figure*}
%\end{landscape}
% \textbf{Scenario 1}\\
% \textbf{Attacker-Type}  attacker is an insider and compromised a node some-how and scanning the network.
% \textbf{Reconnaissance technique}


% \subsubsection{Moving Target Defense}


% \subsection{Security Awareness and Best Practices Against Reconnaissance}
\subsubsection{Game Theory for Deception and MTD}
A game model can play a vital role to increase the uncertainty of adversarial reconnaissance, and also can give different efficient strategies to the defender to implement deception effectively. Deception is an important tactic against adversary reconnaissance, and there are different approaches that apply game-theoretic analysis to cyber deception. The network administrator can introduce deception into response networks scans, such as obscuring certain system characteristics, the game model helps to find defender strategy to implement deception more effectively. Game theory can analyze and develop a solution for decision-making problems among a group of players. It gives quantitative reasoning where the players are either uninformed or unknown about the strategies, moves, and intent of opponents. Therefore, the game model can provide optimal strategies for both defender and attackers to predict the outcome of the deployment of various deception strategies. The Cyber Deception Game represents the Stackelberg game between the defender (e.g., network administrator) and an adversary where the defender moves first and chooses how the systems should respond to scan queries~\cite{schlenker2018deceiving}. A defender can introduce deception by introducing  observed configuration which will hide the true configuration of the network and reduce the attacker's success in reconnaissance phase.

The defender can  protect the true system, from possible exploits and intrusions.\
Each system has certain attributes, e.g., an operating system, a services host, etc. However, when an attacker will view the system it will see the observed configuration which is how a system administrator ought to react to scan requests from an attacker endeavoring to penetrate the system.   Mixed integer linear programming is proved efficient to find strategies of defender against the powerful attacker.  Additionally, greedy algorithm can be used which quickly finds good defender strategies and performs well empirically \cite{schlenker2018deceiving} . Honeypot selection game can leverage the network configuration for a target, by introducing deception game model, the defender can use honeypots in the network in a way so that the attacker will choose to attack honeypots instead of real machines and reduce the chance of correct information gathering in reconnaissance phase.  Probing actions can be used by the attackers, where attackers tried to distinguish which one honeypots from real machines before launching an attack. The probes were noisy, that's why attackers used imperfect information in these models. Using linear programming models for finding the best strategies for the defender to maximize deception strategies can maximize defenders gain in deceiving adversaries in reconnaissance phase Radek Píbil et al.~\cite{pibil2012game}. There are also some works that focused on how to effectively use honeypots (fake systems) as part of a network deception \cite{carroll2011game,wagener2009self,pibil2012game}. 

There has also been a different work on security games that focuses on the role of deception in general to manipulate the beliefs of an attacker~\cite{yin2013optimal,an2011refinement,horak2017manipulating,thakoor2019general}. Finally, to understand the effectiveness of cyber deception and how different research contributed to deploy cyber deception and gain effectiveness in deception game theory can play a predominant role in deceiving attackers at the reconnaissance phases~\cite{ferguson2019game}.

\subsection{Security Awareness and Best Practices}
Security awareness requires both ``knowing'' and ``doing'' the right security actions and measures~\cite{Cybersec84:online}. Most of the security attack is caused by human error (e.g., misconfigured server or database, vulnerable source codes and scripts) and according to the IBM threat landscape of 2018, the human error factor caused 
% \Aron{What is this percentage of?} 
$43\%$ of publicly disclosed misconfiguration incidents~\cite{IBMXForc60:online}. For example, developers can misconfigure a configuration file and leave security holes to be exploited. This is why adversaries can be benefited a lot by performing social engineering techniques. Simple passwords can easily be cracked using brute-force or dictionary attacks. Organizations should provide sufficient security awareness training toward the users and here we discuss a few security best practices:

% \iAron{Most of these do not seem to be connected to reconnaissance. Why are we listing them here? How are they connected to the contributions of this paper?}
% \Shanto{Prof, I've rewritten the items to relate reconnaissance}

% \subsubsection{Security Best Practices against Reconnaissance}
\begin{itemize}
    \item \textbf{Use Strong Password and Passphrase:}
    Many people use weak passwords (e.g., shorter length, words in a dictionary, birth year, mobile number) which is easy to break using Bruteforce or Dictionary attack. Users should use a minimum 8-character length password using numeric values, special symbols (\$, @, \&, \%, etc.), capital and small case letters. Users can also use passphrases that are easier to remember and longer as well. Passphrases are the combination of multiple words separated by ``space'' character (a sentence or a phrase). Strong passwords or passphrases can prevent adversaries to guess or to break potential user credentials.
    
    \item \textbf{Two-Factor Authentication or Two-Step Verification:}
    Users need to maintain two-factor authentication~\cite{jin2004biohashing} or two-step verification~\cite{van2009twostep} while accessing resources or personal accounts. Two-factor authentication requires something users remember (password), something they are (biometric scan, e.g., fingerprint/retina) and something they have (another trusted device, e.g., mobile/computer)~\cite{Twofacto9:online}. On the other hand, two-step verification involves users providing two sequential tokens- first the password, then a One-Time Password (OTP) sent over SMS or email address. Using these security mechanisms prevent unauthorized access even after adversaries extract valuable user credentials.
    
    \item \textbf{Limit BYOD:}
    BYOD stands for Bring Your Own Device. Allowing BYOD in an organization creates opportunities for malicious insiders who can connect an infected device to the internal network. Users can also connect infected pendrives or hard-drives unknowingly in the network. Therefore, organizations can counter the social engineering techniques, \emph{Baiting} and \emph{Reconnaissance by Insider} in particular by limiting the use of personal devices within the network. 
    
    \item \textbf{Utilize IDS and IPS:}
    Organizations should introduce intrusion detection and prevention systems to identify typical penetration in the network. Host-based IDS and Network-based IDS are the most common detection systems. HIDS can mitigate the risk of local discovery techniques in a compromised host by identifying the presence of an attacker. On the other hand, NIDS can mitigate and slow down the adversary's approach while performing network scanning techniques. Honeypots can be utilized as well by deploying it within the network with particular configurations. 
    
    \item \textbf{Enforce Firewall Rules:}
    Organizations need to enforce certain firewall rules that block particular scanning packets (TCP/UDP/ICMP) and mitigate the network-based reconnaissance techniques. Organizations should use both hardware and software-based firewalls as a security measure. Hardware firewalls are typically used to protect a network and are deployed at the entrance of the network (e.g., a gateway). Software firewalls are installed in a device protecting it from other internal or external nodes. Typical rules can avoid particular ICMP, TCP, and UDP network scan requests.
    
    \item \textbf{Isolate Zones:}
    Dividing the whole network into separate zones can block and slow down adversaries to have a whole picture of the network. Isolated zones are useful in case BYOD is allowed in an organization and can easily be adapted to cyber deception and moving target defense. Therefore, even a device is compromised adversaries cannot have the whole picture of the entire organizational network.
    
    \item \textbf{Resource Access Control:}
    Organizations should maintain proper access controls to resources in terms of both physical and network-based access. Proper access control can slow down the adversaries while performing internal scanning and discoveries.
    
    \item \textbf{Vulnerability Inspection:}
    Organizations are often (e.g., each month) required to inspect vulnerabilities within the system to identify any misconfiguration or security holes. Performing SWOT (Strength-Weakness-Opportunity-Threat) analysis on regular-basis can mitigate the effectiveness of reconnaissance at different levels and phases.
    
    \item \textbf{Update Patches:}
    Regular update of patches can mitigate the effect of vulnerability scanning. Organizations should keep all the security measures (e.g., security softwares/antivirus) up-to-date to minimize vulnerability exposure and discovery techniques in the local machine.
    
    \item \textbf{File Encryption:}
    As adversaries are capable of accessing files, users should encrypt files containing confidential information in order to keep information secure and safe. Encrypting files and directories can mitigate local file discovery techniques.
    
    % \item \textbf{Run SWOT Analysis:}
    % Organizations should run a SWOT analysis in all parts of it's structure and products. SWOT stands for \emph{Strengths}, \emph{Weaknesses}, \emph{Opportunities}, and  \emph{Threats}. The analysis can essentially reduce the risk factors.
    
\end{itemize}

Security awareness and best practices can mitigate the adversarial reconnaissance at a good level. As reconnaissance is the prerequisite part of any further progress made by adversaries, defenders are required to take necessary measures that prevent or mitigate the effect of recon techniques.

\vspace{3mm}
Table~\ref{tab: defensive_measurements} presents which different defensive measures can counter particular reconnaissance techniques. In this table, we see that \emph{Social Engineering}, \emph{Network Scanning}, and \emph{Local Discovery} techniques can be detected and thus be prevented with effective measures. \emph{Deception} and \emph{MTD}-based techniques can mitigate adversarial scanning and local discovery techniques. Above all, security awareness (through employee training programs) and known best practices can effectively mitigate adversarial techniques to a diverse extent.

\begin{table}[!ht]
\centering
\caption{Defensive Measures against Reconnaissance Techniques}
\label{tab: defensive_measurements}
\begin{tabular}{|c|c|c|c|c|}
\hline
\diagbox[width=15em]{Measures}{Techniques}     & \begin{tabular}[c]{@{}c@{}}Target\\ Footprinting\end{tabular} & \begin{tabular}[c]{@{}c@{}}Social \\ Engineering\end{tabular} & \begin{tabular}[c]{@{}c@{}}Network\\ Scanning\end{tabular} & \begin{tabular}[c]{@{}c@{}}Local\\ Discovery\end{tabular} \\ \hline\hline
Reconnaissance Detection & \textbf{\textsf{X}} & \checkmark & \checkmark & \checkmark \\\hline
Cyber Deception/MTD   &  \textbf{\textsf{X}}   &  \textbf{\textsf{X}} &  \checkmark & \checkmark \\ \hline
Security Awareness and Best Practices & \checkmark  & \checkmark &  \checkmark &  \checkmark \\ \hline
\end{tabular}
\end{table}




% \subsection{Discussion}

% \iAron{We should merge this paragraph into the conclusion.}

% \Aron{`We find that...'}






==> tables/host_info_discovery.tex <==
\begin{table}[htbp]
\centering
\caption{Host System Information Discovery}
\label{tab:host_domain}
\begin{tabular}{|l|l|l|}
\hline
Info Discovery                                                                             & Target Info                                                        & Reported APT(Procedures/Groups)                                                                                                                                                                                             \\ \hline\hline

\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}File and\\Directory\end{tabular}}   & \begin{tabular}[c]{@{}l@{}}Directory \&\\ File Lists\end{tabular}      & \begin{tabular}[c]{@{}l@{}} 4H RAT, ADVSTORESHELL, APT18/3/32, BBSRAT, Brave Prince, Cannon,\\China Chopper, Crimson, Derusbi, Gold Dragon, HTTPBrowser etc.  etc.\end{tabular} \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}} Search\\Ability \end{tabular} & \begin{tabular}[c]{@{}l@{}} CORALDECK, Denis, FALLCHILL, Kasidet, Ke3chang, KEYMARBLE,\\ Linfo, NETEAGLE, OceanSalt, PinchDuke, RedLeaves etc. \end{tabular} \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}} Specific\\extensions \end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}} Azorult, BADNEWS, BadPatch, CHOPSTICK, CosmicDuke, Crimson, Forfiles,\\ GravityRAT, PinchDuke, Prikormka, Pteranodon, Rover, TrickBot etc   \end{tabular}  \\ \hline
                                                                                           
\multirow{4}{*}{Process}   & \begin{tabular}[c]{@{}l@{}}Process\\List\end{tabular}      & \begin{tabular}[c]{@{}l@{}} 4H RAT, ADVSTORESHELL, APT1/3/37, Azorult, Cannon, Carbon,\\Crimson, DarkComet, ELMER, FELIXROOT etc.\end{tabular} \\ \cline{2-3} 
                                                                                           &  Process ID & \begin{tabular}[c]{@{}l@{}} Bankshot, ChChes, Derusbi, Pupy etc. \end{tabular} \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}} Environment\\variable \end{tabular}                                                          & GeminiDuke  \\ \hline
                                                                                          
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Peripheral\\Devices\end{tabular}}   & USB Devices     & \begin{tabular}[c]{@{}l@{}} APT 28, BADNEWS, BlackEnergy, Gamaredon Group, USBStealer etc.\end{tabular} \\ \cline{2-3} 
                                                                                           & BT Devices & APT 37 \\ \cline{2-3} 
                                                                                           &  Smart Card  & FlawedAmmyy, RTM etc.  \\ \hline
                                                                                           
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Registry\\Information\end{tabular}}   & \begin{tabular}[c]{@{}l@{}}Registry keys\\and Values\end{tabular}      & \begin{tabular}[c]{@{}l@{}} Carbon, Denis, Derusbi, Epic, InvisiMole,\\WINDSHIELD, Zeus Panda etc.\end{tabular} \\ \cline{2-3} 
                                                                                           &  \begin{tabular}[c]{@{}l@{}}Installed\\Software\end{tabular} & \begin{tabular}[c]{@{}l@{}} Azorult, Stealth Falcon, Ursnif etc. \end{tabular} \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}} Miscellaneous\\system info \end{tabular}                                                          & APT32, HOPLIGHT, Hydraq, ROKRAT etc  \\ \hline
                                                                                           
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Hardware and\\Platform\end{tabular}}   & OS Version      & \begin{tabular}[c]{@{}l@{}} 4H RAT, APT32, Azorult, BadPatch, BlackEnergy,\\Cannon, CORESHELL, Epic, FELIXROOT, Hydraq, jRAT etc.\end{tabular} \\ \cline{2-3} 
                                                                                           &  \begin{tabular}[c]{@{}l@{}}OS\\Architecture\end{tabular} & \begin{tabular}[c]{@{}l@{}} Cardinal RAT, Darkhotel, Empire, FELIXROOT, HAWKBALL, KONNI,\\ Patchwork, POWERSTATS, Pupy etc. \end{tabular} \\ \cline{2-3} 
                                                                                            &  \begin{tabular}[c]{@{}l@{}}Drive\\Information\end{tabular} & \begin{tabular}[c]{@{}l@{}} Cannon, HOPLIGHT, InnaputRAT, InvisiMole, JHUHUGIT, Kazuar, \\ KONNI, MoonWind, NOKKI, Octopus, Proxysvc etc. \end{tabular} \\ \cline{2-3}
                                                                                            &  \begin{tabular}[c]{@{}l@{}}BIOS\\Information\end{tabular} & \begin{tabular}[c]{@{}l@{}} APT37, BlackEnergy, HALFBAKED, RogueRobin etc. \end{tabular} \\ \cline{2-3}
                                                                                            
                                                              &  \begin{tabular}[c]{@{}l@{}}Peripheral\\Devices\end{tabular} & \begin{tabular}[c]{@{}l@{}} Agent Tesla, Azorult, Shamoon, SynAck etc. \end{tabular} \\ \cline{2-3}
                                                                                           & \begin{tabular}[c]{@{}l@{}} CPU\\architecture \end{tabular}                                                          & Cardinal RAT, Darkhotel, FELIXROOT, Final1stspy, Remsec etc  \\ \hline
                                                                                           
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}System\\Services\end{tabular}}   & Service List     & \begin{tabular}[c]{@{}l@{}} Epic, GravityRAT, JPIN, Kwampirs, TrickBot etc.\end{tabular} \\ \cline{2-3} 
                                            & Configuration & BBSRAT, GeminiDuke, HyperBro etc. \\ \hline
                                                                                           
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Network\\ Configuration\end{tabular}}  & \begin{tabular}[c]{@{}l@{}} Local IP\\ Address \end{tabular} & \begin{tabular}[c]{@{}l@{}}admin@338, Agent Tesla, APT1/3/19/32, Astaroth, BlackEnergy,\\ Carbon, ipconfig, ifconfig, Mosquito, MuddyWater, NanoCore, Reaver etc.\end{tabular} \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}}Public IP\\ Address\end{tabular} & KeyBoy                                                                                                                                                                                                            \\ \cline{2-3} 
                                                                                           & Mac Addr  & \begin{tabular}[c]{@{}l@{}}APT3/19, Catchamas, Crimson, FALLCHILL, GravityRAT, InvisiMole,\\Magic Hound, Revenge RAT, T9000,  \end{tabular}                                                                                                              \\ \cline{2-3} 
                                                                                           & Open Ports & BlackEnergy, HDoor etc \\\cline{2-3}
                                                                                           & WINS & Agent.btz, APT3, Lazarus Group\\\cline{2-3}
                                                                                           & DHCP & Agent.btz, APT3, FELIXROOT, ifconfig, ipconfig, Lazarus Group\\\cline{2-3}
                                                                                           & DNS & Agent.btz,Empire, ifconfig, ipconfig, JPIN, Remsec \\\hline

\multirow{4}{*}{Security Software}                                                         & \begin{tabular}[c]{@{}l@{}}Antivirus\\ Detection\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Astaroth, CHOPSTICK, Empire, EvilBunny, FELIXROOT, Flame,\\ Mosquito, Patchwork, StoneDrill, StreamEx, T9000, Comnie, CozyCar,\\ Crimson, Darkhotel, DustySky, Exaramel etc.\end{tabular} \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}}Forensic tools\\ Detection\end{tabular} & CHOPSTICK                                                                                                                                                                                                              \\ \cline{2-3} 
                                                                                           & Firewall                                                           & \begin{tabular}[c]{@{}l@{}}FELIXROOT, jRAT, Micropsia, Naikon, netsh, StreamEx, Zeus Panda\end{tabular}                                                                                                              \\ \cline{2-3} 
                                                                                           & Sandbox                                                            & FIN8                                                                                                                                                                                                                   \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Virtualization/\\ Sandbox Evasion\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Virtual\\ Environment\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} BadPatch, CHOPSTICK, CozyCar, FinFisher, GravityRAT,\\ OopsIE, Pupy, RogueRobin, yty, UBoatRAT \end{tabular}  \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}}Sandbox\\ Environment\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} CozyCar, Dyre, EvilBunny, FIN7, FinFisher, Remcos, ROKRAT,\\ StoneDrill, SynAck, Ursnif, yty  \end{tabular}  \\ \hline
\end{tabular}
\end{table}

==> tables/net_info_discovery.tex <==
\begin{table}[htbp]
\centering
\caption{Information Discovery at Network Domain}
\label{tab:network_domain}
\begin{tabular}{|l|l|l|}
\hline
Info Discovery                                                                             & Target Info                                                        & Reported APT(Procedures/Groups)                                                                                                                                                                                              \\ \hline\hline
                                                                                           
Network Connection & \begin{tabular}[c]{@{}l@{}}Reachable\\IP Hosts\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} APT1/3/32, BlackEnergy, Carbon, Empire, Epic, jRAT,\\ Ke3chang, netstat, PlugX, Pupy, Remsec, Zebrocy etc. \end{tabular}  \\ \hline
                                                                                           
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}} Network Service\\ Scanning \end{tabular}} & \begin{tabular}[c]{@{}l@{}}Open Ports\\ Scanning\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} APT32/39, Cobalt Strike, Empire,  HDoor, Koadic, menuPass,\\ MURKYTOP, Pupy, Remsec, SpeakUp, Suckfly,\\ Tropic Trooper, Xbash, XTunnel etc \end{tabular}  \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}}Network\\Services\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} APT32, Leafminer, Threat Group-3390 etc.  \end{tabular}  \\ \cline{2-3}
                                                                                           & \begin{tabular}[c]{@{}l@{}}OS\\fingerprinting \end{tabular} & APT32\\ \cline{2-3}
                                                                                           & \begin{tabular}[c]{@{}l@{}} Active\\ Directory,\\SQL Server,\\NetBIOS \end{tabular} & FIN6 \\ \hline
                                                                                           
                                                                                           
Remote System & \begin{tabular}[c]{@{}l@{}}Available\\ Nodes or\\ servers\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} APT3/32, Carbon, Cobalt Strike, FIN5/6/8, menuPass, MURKYTOP,\\ njRAT, Nltest, Ping, Remsec, Sykipot, Threat Group-3390, WannaCry etc. \end{tabular}  \\ \hline

\multirow{2}{*}{Network Sniffing} & credentials  &  \begin{tabular}[c]{@{}l@{}} APT28/33, Regin, Responder, Stolen Pencil etc. \end{tabular}  \\ \cline{2-3} 
                                                                                           & \begin{tabular}[c]{@{}l@{}}Configuration\\ Details\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} APT28, Empire, PoshC2, Responder etc.  \end{tabular}  \\ \hline
\multirow{3}{*}{Network Share} & \begin{tabular}[c]{@{}l@{}}Shared\\ Drive\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} Cobalt Strike, Empire, Net, Pupy, Sowbug, Zebrocy etc. \end{tabular}  \\ \cline{2-3} 
                                                                                   & \begin{tabular}[c]{@{}l@{}}Share in\\remote host\end{tabular}         &  MURKYTOP \\ \cline{2-3}
                                                                                           & \begin{tabular}[c]{@{}l@{}}Network\\ Share list\end{tabular}      &  \begin{tabular}[c]{@{}l@{}} APT1, Kwampirs, Pupy, Sowbug etc.  \end{tabular}  \\ \hline
\end{tabular}
\end{table}

==> tables/scanning_techniques.tex <==
% \begin{table}[htb]
%     \caption{Scanning Steps, Techniques, and Tools}
%     \label{tab:scanning}
%     \centering
%     \begin{threeparttable}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{|M{2cm}|M{4cm}|M{1.2cm}|M{3cm}|M{1.4cm}|M{4cm}|}
%         \hline
%         Steps & Techniques & Type  & Target Information & Phase & Tools \\ \hline \hline
%         \multirow{4}{1.8cm}{} & ICMP / TCP / UDP Scanning   & Active  & locating active devices, firewall configuration & Internal / External &  NMap\tnote{1}
%         % \cite{NmaptheN26:online}
%         % \cite{lyon2009nmap} 
%         \\ \cline{2-6}
%         Scanning Active Hosts & Ping Sweep & Active  & live hosts within a range of IP addresses & Internal / External & NMap, Angry IP scanner\tnote{2}\space,
%         % \cite{AngryIPS41:online} 
%         Solarwinds tools\tnote{3}
%         % \cite{NetworkM19:online}
%         \\ \cline{2-6}
%         & ARP Scanning & Active & live hosts in a LAN & Internal & ARP Ping\tnote{4}
%         % ~\cite{ARPPingT52:online}
%         \\\cline{2-6}
%         & Sniffing Packets (Source / Destination Address) & Passive  & live hosts in internal or external network & Internal / External & Wireshark, Ettercap\tnote{5} 
%         % \cite{Ettercap73:online}
%         \\ \hline
        
%         \multirow{2}{1.8cm}{\begin{tabular}[c]{@{}c@{}}Scanning\\Open Ports\end{tabular}} & Custom packets using TCP flags (SYN/ACK/FIN scan, stealth scan, XMAS scan, NULL scan, IDLE scan) & Active  & open TCP ports, firewall and networks test result & Internal / External & NMap, Hping2
%         % \cite{kamerling2012hping2}
%         / Hping3\tnote{6}\space,
%         % \cite{HpingAct62:online}, 
%         Amap\tnote{7}\space,
%         % \cite{AmapPene25:online}, 
%         SuperScan\tnote{8}
%         % \cite{Supersca89:online}
%         \\ \cline{2-6}
%         & UDP Scan & Active & open UDP ports and services (e.g., DNS, VPN, SNMP) & Internal / External & Nmap\\\hline
        
%         \multirow{3}{1.8cm}{} & Banner grabbing and OS fingerprinting by sending crafted packets and analyzing responses & Active  & \multirow{2}{2.5cm}{\begin{tabular}[c]{@{}c@{}}OS /\\ application /\\ service version,\\ TCP/IP stack\end{tabular}} & Internal / External & Telnet,
%         % ~\cite{postel1983telnet}, 
%         NetCraft, IDServe\tnote{9} ,
%         % \cite{GRCIDSer27:online}, 
%         Nmap, Winfingerprint\tnote{10} \space, 
%         % \cite{Winfinge64:online}
%         % \cite{ganesan2004tcp},  
%         Xprobe2\tnote{11}
%         % \cite{arkin2003present} 
%         \\ \cline{2-3}\cline{6-6}
%         Scanning Vulnerability & Banner grabbing and OS fingerprinting using sniffing techniques & Passive & & & Ettercap,
%         % \cite{norton2004ettercap}, 
%         P0f\tnote{12} \space,
%         % \cite{p0fv377:online}, 
%         NetworkMiner\tnote{13} \space,
%         % \cite{hjelmvik2008passive}, 
%         NetSleuth\tnote{14} ,
%         % \cite{Security52:online}, 
%         PRADS\tnote{15} \space\space,
%         % \cite{gamelinu62:online}, 
%         SATORI\tnote{16} ,
%         % \cite{xnihsato58:online}
%         \\ \cline{2-6}
        
%          & 
%         %  \iAron{how? this field should describe the ``Techniques'', not the objective} 
%         %  Find application / service vulnerabilities, configuration errors
%         Fingerprinting and patch-level assessment & Active / Passive  & application / OS / service vulnerability identification & Internal / External & Nessus,
%         %  ~\cite{beale2004nessus}, 
%          Saint\tnote{17} \space ,
%         %  \cite{Penetrat18:online}, 
%          Cisco-Torch\tnote{18} \space\space 
%         %  \cite{ciscotor71:online} 
%          and other vulnerability scanning tools\\ \hline
        
%         % Design Network Diagram & Network discovery & Active/ Passive  & Network view & Internal/ External & LANsurveyor (replaced by Network Topology Mapper \cite{LANSurve74:online}), CartoReso, traceroute, NeoTrace \cite{NeoTrace68:online} etc and other online network mappers\\ \hline
  
%     \end{tabular}
%     }
%     \begin{tablenotes}
%     \footnotesize
%      \item[1] \url{https://nmap.org/}
%      $^2$ \url{https://angryip.org/}
%      $^3$ \url{https://www.solarwinds.com/engineers-toolset/use-cases/network-monitoring-tools}\\
%      $^4$ \url{https://www.netscantools.com/nstpro_arpping.html}
%      $^5$ \url{https://www.ettercap-project.org/}
%      $^6$ \url{http://www.hping.org/}\\
%      $^7$ \url{https://tools.kali.org/information-gathering/amap}
%      $^8$ \url{https://sectools.org/tool/superscan/}
%      $^9$ \url{https://www.grc.com/id/idserve.htm}\\
%      $^{10}$ \url{https://securiteam.com/tools/5HP0A1P2LK/}
%      $^{11}$ \url{https://github.com/binarytrails/xprobe2}
%      $^{12}$ \url{http://lcamtuf.coredump.cx/p0f3/\#}\\
%      $^{13}$ \url{https://www.netresec.com/?page=networkminer}\\
%      $^{14}$ \url{https://www.securitywizardry.com/products/scanning-products/wireless-tools/netsleuth}\\
%      $^{15}$ \url{https://github.com/gamelinux/prads}
%      $^{16}$ \url{https://github.com/xnih/satori}\\
%      $^{17}$ \url{https://www.saintcorporation.com/products/penetration-testing/}
%      $^{18}$ \url{https://tools.kali.org/information-gathering/cisco-torch}
%   \end{tablenotes}
%     \end{threeparttable}
% \end{table}





\begin{table}[htb]
    \caption{Scanning Techniques and Tools}
    \label{tab:scanning}
    \centering
    \begin{threeparttable}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|M{2cm}|M{4cm}|M{1.2cm}|M{3cm}|M{1.4cm}|M{4cm}|}
        \hline
        Steps & Techniques & Type  & Target Information & Phase & Tools \\ \hline \hline
        \multirow{4}{1.8cm}{} & ICMP / TCP / UDP Scanning   & Active  & {Network View/Security} & Internal / External &  NMap\tnote{1}
        % \cite{NmaptheN26:online}
        % \cite{lyon2009nmap} 
        \\ \cline{2-6}
        Scanning Active Hosts & Ping Sweep & Active  & {Network View} & Internal / External & NMap, Angry IP scanner\tnote{2}\space,
        % \cite{AngryIPS41:online} 
        Solarwinds tools\tnote{3}
        % \cite{NetworkM19:online}
        \\ \cline{2-6}
        & ARP Scanning & Active & {Network View} & Internal & ARP Ping\tnote{4}
        % ~\cite{ARPPingT52:online}
        \\\cline{2-6}
        & Sniffing Packets (Source / Destination Address) & Passive  & {Network View} & Internal / External & Wireshark, Ettercap\tnote{5} 
        % \cite{Ettercap73:online}
        \\ \hline
        
        \multirow{2}{1.8cm}{\begin{tabular}[c]{@{}c@{}}Scanning\\Open Ports\end{tabular}} & Custom packets using TCP flags (SYN/ACK/FIN scan, stealth scan, XMAS scan, NULL scan, IDLE scan) & Active  & {System Services, Network Security} & Internal / External & NMap, Hping2
        % \cite{kamerling2012hping2}
        / Hping3\tnote{6}\space,
        % \cite{HpingAct62:online}, 
        Amap\tnote{7}\space,
        % \cite{AmapPene25:online}, 
        SuperScan\tnote{8}
        % \cite{Supersca89:online}
        \\ \cline{2-6}
        & UDP Scan & Active & {DNS and Reachable Hosts, System Services} & Internal / External & Nmap\\\hline
        
        \multirow{3}{1.8cm}{} & Banner grabbing and OS fingerprinting by sending crafted packets and analyzing responses & Active  & \multirow{2}{2.8cm}{\begin{tabular}[c]{@{}c@{}}{System/Service}\\{Configurations,}\\ {Running Applications,}\\ {Versions}\end{tabular}} & Internal / External & Telnet,
        % ~\cite{postel1983telnet}, 
        NetCraft, IDServe\tnote{9} ,
        % \cite{GRCIDSer27:online}, 
        Nmap, Winfingerprint\tnote{10} \space, 
        % \cite{Winfinge64:online}
        % \cite{ganesan2004tcp},  
        Xprobe2\tnote{11}
        % \cite{arkin2003present} 
        \\ \cline{2-3}\cline{6-6}
        Scanning Vulnerability & Banner grabbing and OS fingerprinting using sniffing techniques & Passive & & & Ettercap,
        % \cite{norton2004ettercap}, 
        P0f\tnote{12} \space,
        % \cite{p0fv377:online}, 
        NetworkMiner\tnote{13} \space,
        % \cite{hjelmvik2008passive}, 
        NetSleuth\tnote{14} ,
        % \cite{Security52:online}, 
        PRADS\tnote{15} \space\space,
        % \cite{gamelinu62:online}, 
        SATORI\tnote{16} ,
        % \cite{xnihsato58:online}
        \\ \cline{2-6}
        
         & 
        %  \iAron{how? this field should describe the ``Techniques'', not the objective} 
        %  Find application / service vulnerabilities, configuration errors
        Fingerprinting and patch-level assessment & Active / Passive  & {Host / Network / Application Vulnerabilities} & Internal / External & Nessus,
        %  ~\cite{beale2004nessus}, 
         Saint\tnote{17} \space ,
        %  \cite{Penetrat18:online}, 
         Cisco-Torch\tnote{18} \space\space 
        %  \cite{ciscotor71:online} 
         and other vulnerability scanning tools\\ \hline
        
        % Design Network Diagram & Network discovery & Active/ Passive  & Network view & Internal/ External & LANsurveyor (replaced by Network Topology Mapper \cite{LANSurve74:online}), CartoReso, traceroute, NeoTrace \cite{NeoTrace68:online} etc and other online network mappers\\ \hline
  
    \end{tabular}}
    \begin{tablenotes}
    \footnotesize
     \item[1] \url{https://nmap.org/}
     $^2$ \url{https://angryip.org/}
     $^3$ \url{https://www.solarwinds.com/engineers-toolset/use-cases/network-monitoring-tools}\\
     $^4$ \url{https://www.netscantools.com/nstpro_arpping.html}
     $^5$ \url{https://www.ettercap-project.org/}
     $^6$ \url{http://www.hping.org/}\\
     $^7$ \url{https://tools.kali.org/information-gathering/amap}
     $^8$ \url{https://sectools.org/tool/superscan/}
     $^9$ \url{https://www.grc.com/id/idserve.htm}\\
     $^{10}$ \url{https://securiteam.com/tools/5HP0A1P2LK/}
     $^{11}$ \url{https://github.com/binarytrails/xprobe2}
     $^{12}$ \url{http://lcamtuf.coredump.cx/p0f3/\#}\\
     $^{13}$ \url{https://www.netresec.com/?page=networkminer}\\
     $^{14}$ \url{https://www.securitywizardry.com/products/scanning-products/wireless-tools/netsleuth}\\
     $^{15}$ \url{https://github.com/gamelinux/prads}
     $^{16}$ \url{https://github.com/xnih/satori}\\
     $^{17}$ \url{https://www.saintcorporation.com/products/penetration-testing/}
     $^{18}$ \url{https://tools.kali.org/information-gathering/cisco-torch}
   \end{tablenotes}
    \end{threeparttable}
\end{table}

==> tables/user_info_discovery.tex <==
\begin{table}[htbp]
\centering
\caption{User Information Discovery}
\label{tab:user_domain}
\begin{tabular}{|M{3.2cm}|M{3.2cm}|M{8cm}|}
\hline
Info Discovery   & Target Info   & Reported APT(Procedures/Groups) \\ \hline\hline     
\multirow{4}{*}{User and Group Info} & Local User Account      &  admin@338, Agent Tesla, APT1, dsquery, Empire, GeminiDuke, OSInfo, PoshC2, Pupy etc. \\ \cline{2-3} 
 & Domain User  & Bankshot, dsquery, Empire, OilRig, OSInfo, PoshC2 etc. \\ \cline{2-3}
  & Group info & APT1/3/32, Carbon, Kazuar, OilRig, Pupy, Sykipot etc.\\ \hline
\multirow{2}{*}{Browser Bookmark} &  Bookmarks and History  &  Calisto, Empire, MobileOrder etc.  \\ \cline{2-3} 
 & User Profile  &  Machete   \\ \hline                      
Password Policy & Policy &  Kwampirs, Net, OilRig, PoshC2 etc. \\  \hline
\end{tabular}
\end{table}

